$\nabla^2$DFT: A Universal Quantum Chemistry Dataset of Drug-Like Molecules and a Benchmark for Neural Network Potentials

Methods of computational quantum chemistry provide accurate approximations of molecular properties crucial for computer-aided drug discovery and other areas of chemical science. However, high computational complexity limits the scalability of their applications. Neural network potentials (NNPs) are a promising alternative to quantum chemistry methods, but they require large and diverse datasets for training. This work presents a new dataset and benchmark called $\nabla^2$DFT that is based on the nablaDFT. It contains twice as much molecular structures, three times more conformations, new data types and tasks, and state-of-the-art models. The dataset includes energies, forces, 17 molecular properties, Hamiltonian and overlap matrices, and a wavefunction object. All calculations were performed at the DFT level ($\omega$B97X-D/def2-SVP) for each conformation. Moreover, $\nabla^2$DFT is the first dataset that contains relaxation trajectories for a substantial number of drug-like molecules. We also introduce a novel benchmark for evaluating NNPs in molecular property prediction, Hamiltonian prediction, and conformational optimization tasks. Finally, we propose an extendable framework for training NNPs and implement 10 models within it.

==> 05_methods.tex <==
% --------------  original methods description
%The goal of this benchmark is to advance and standardize studies in the field of machine learning methods for the DFT problem solution. Therefore, we focus on the class of models able to predict quantum chemistry properties, especially electron densities, wave functions, and other \TODO{?}. However, most of these methods can be naturally adapted to predict basic integral properties of a molecular conformation such as potential energy of a given conformation.
% 

%We compare models in two different settings: 
%\begin{itemize}
%    \item conformational energy prediction and
%    \item quantum properties prediction.
%\end{itemize}

The goal of this benchmark is to advance and standardize studies in the field of machine learning methods for computational quantum chemistry.
We focus on the class of models that predict quantum chemistry properties from the spatial representation of molecules.
\art{More precisely, we study models for three tasks: conformational energy and atomic forces prediction, DFT Hamiltonian prediction, and conformational geometry optimization.
To solve these task, we employ neural networks $f(s; \bm{\theta})$ parametrized by weights $\bm{\theta}$.}

\paragraph*{Conformational energy and atomic forces prediction.}
\art{We denote the energy predicted by a certain method for conformation $s$ as $E^{\text{oracle}}_s$,
where the superscript "oracle" refers to different methodologies for solving the Schr{\"o}dinger equation, such as DFT-based approaches with different levels of theory.
For the task of conformational energy and atomic forces prediction, we consider the neural network to take conformation $s$ as an input and output energy $\hat{E}_s = f(s; \bm{\theta})$, $f(s; \bm{\theta}):~\{\bm{z}, \bm{X}\} \rightarrow \mathbb{R}$.
To predict the interatomic forces, we take the gradients of $\hat{E}_s$ w.r.t. coordinates of atoms $\bm{X}$:}
\art{
\begin{equation}
    \hat{\bm{F}}_s = \frac{\partial f(s;\bm{\theta})}{\partial \bm{X}}.
\end{equation}
}
\art{
The neural networks are trained to minimize $L_1$ or $L_2$ loss for energy and interatomic forces.
We evaluate models on $D^{\text{structure}}, D^{\text{scaffold}}, D^{\text{conformation}}$ using Mean Absolute Error (MAE) as metrics.
}

\art{
\begin{equation}
    MAE^D_E = \frac{1}{|D|}\sum_{s \in D}|\hat{E}_s - E_s|
\end{equation}
}

\paragraph*{DFT Hamiltonian prediction.}
\kuz{
The neural networks are trained to minimize $L_1$ or $L_2$ loss for the Hamiltonian matrix (all models), overlap matrix (PhiSNet and SchNOrb), and energy (SchNOrb).
We evaluate models on $D^{\text{structure}}, D^{\text{scaffold}}, D^{\text{conformation}}$ using Mean Absolute Error (MAE) as metrics.
}

\kuz{
\begin{equation}
    MAE^D_E = \frac{1}{|D|}\sum_{s \in D} \frac{1}{n_s^2}\sum_{i,j}|\hat{H}^{ij}_s - H^{ij}_s|,
\end{equation}
where $n_s$ is the number of electronic orbitals for a sample $s$.
}
\paragraph*{Conformational geometry optimization.}
\art{We establish a novel benchmark for conformational geometry optimization.
Specifically, we consider }

\begin{figure}[!t]
    \includegraphics[width=\linewidth]{./images/scheme.pdf}
    \caption{High-level architecture of the models.}
    \label{fig:genarch}
\end{figure}

Figure~\ref{fig:genarch} shows a bird's eye overview of the general architecture for the models that we compare in this work. It consists of four main blocks:
\begin{itemize}
    \item \emph{inputs}: all considered models use atom types, coordinates, or their functions as input;
    \item \emph{embedding layers}: MLP or a single Linear layer;
    \item \emph{interaction layers}: this is usually the main part with model-specific architecture;
    \item \emph{output layers}: depending on the model, output layers are designed to convert internal representations into specific desired values.
\end{itemize}


\subsection{Linear Regression}\label{ssec:lr}
We propose the linear regression model (LR) as a simple baseline for molecular properties prediction, in particular energy prediction.
It takes the numbers of each atom type in the molecule as an input representation and predicts energy as its weighted sum. 
While it is clear that more sophisticated handcrafted features may increase a model's accuracy and generalization power, this work focuses on deep models that can learn such features automatically.

\subsection{SchNet \texorpdfstring{\cite{schnet2017}}{}}\label{ssec:schnet}
The \emph{SchNet} model was one of the first works that suggested a neural architecture for atomic forces and molecular energy prediction. The key contribution here is the \emph{cfconv}, a continuous-filter convolutional layer for modeling objects with arbitrary positions.
The model is schematically represented in Figure~\ref{fig:schnet}.

\begin{figure}[!t]
    \includegraphics[width=\linewidth]{./images/schnet/all.pdf}
    \caption{A schematic depiction of the \emph{SchNet} architecture with its sub-units. The left column shows an overview and the middle and right columns detail the \emph{Interaction} and \emph{cfconf} blocks. $X$ is an atom's representation, $D_{ij}$ is the pairwise distance matrix. Atom-wise blocks are multilayer perceptrons applied to each atom representation independently.}
    \label{fig:schnet}
\end{figure}

Given feature representations of $n$ objects $X^l = (x_1, x_2, ..., x_n) \in \mathbb{R}^F$ (at layer $l$), which are at positions $R = (r_1, ..., r_n) \in \mathbb{R}^D$, and a special function $W^l$ that maps $R$'s domain to $X$'s domain, i.e., $W^l: \mathbb{R}^D \rightarrow \mathbb{R}^F$, the output of the proposed \emph{cfconv} layer is defined as

$$x_i^{l+1} = (X^l * W^l)_i = \sum_{j} x_j^l \circ W^l (r_i - r_j).$$
where $\circ$ denotes element-wise multiplication.

The use of \emph{cfconv} and the overall network architecture design ensure an important property: energy and force predictions are rotationally invariant and equivariant, respectively. For instance, in the \emph{cfconv} layer $W^l$ is a combination of $||r_i-r_j||$, radial basis functions, dense feedforward layers, and a shifted \emph{softplus} activation function $\mathrm{ssp}(x) = \ln(0.5 e^{x} + 0.5)$.

The model takes nuclear charges and atomic positions as inputs. Nuclear charges are first embedded into 64-dimensional representations, After that, they are processed with an ``Interaction'' block of layers that includes $3$ applications of \emph{cfconv} (cf. Fig.~\ref{fig:schnet}, thus enriching the feature representation with positional information. Then more atom-wise modifications follow to be pooled in a final layer to obtain the energy prediction. Differentiating the energy with respect to atom positions yields the forces, hence force predictions can be and are also added to the loss function. 

The resulting method has been tested on three datasets: QM9~\cite{ruddigkeit2012enumeration,ramakrishnan2014quantum}, MD17~\cite{chmiela2017machine}, and ISO17 (introduced in the original work\cite{schnet2017}). For more details, we refer to~\citet{schnet2017}.

\subsection{PaiNN}\label{ssec:painn}
The PaiNN (polarizable atom interaction neural network) model~\citep{schutt2021equivariant} may be considered a rotationally equivariant successor of the SchNet model.
The main contribution of this work is the extension of an internal representation with an equivariant vector counterpart and the introduction of the equivariant message function, which takes invariant and equivariant features and predicts an update of the vector part. Such a model can propagate directional information in the message-passing steps.
The model consists of an initial embedding block, several message and update blocks, and an output block. \\
In the message block, a features-wise update of invariant and equivariant features  is predicted.

\begin{align}
    \Delta x_i^m &= \left( X* W_x \right)_i = \sum_{j} x_j^l \circ W_x \left( \lVert r_i - r_j \rVert \right); \\
    \begin{split}
        \Delta v_i^{m}  &= \sum_{j} v_j \circ \phi_{vv}(x_j) \circ W_{vv} \left( \lVert r_i - r_j \rVert \right) \\
        &+ \sum_{j}  \phi_{vx}(x_j) \circ W’_{vs} \left( \lVert r_i - r_j \rVert \right) \frac{r_i - r_j}{\lVert r_i - r_j \rVert}.
    \end{split}
\end{align}

In the update block, atom-wise updates of invariant and equivariant features are predicted.


\begin{align}
    \begin{split}
        \Delta x_i^{u} &= a_{xx}\left( x_i, \lvert V v_i\rVert \right) \\
        &+ a_{xv} \left( x_i, \lVert V v_i \rVert \right) \langle U v_i, V v_i \rangle ;
    \end{split} \\
   \Delta v_i^u &= a_{vv}\left( v_i, \lVert V v_i \rVert \right) U v_i .
\end{align}

\subsection{DimeNet~\texorpdfstring{\cite{gasteiger2021directional}}{}}

A major contribution of \emph{DimeNet} is that it takes into account not only the distances between pairs of atoms but also angles formed by triples of atoms. The authors note that the pairwise distance matrix is sufficient to describe the full geometric information of the molecule. However, in order to keep computational costs reasonable, graph neural networks (GNNs) ignore connections between atoms that are more than a certain cutoff distance apart. One possible result of this simplification could be that the GNN would not be able to distinguish between some molecules.

\begin{figure}[!t]
    \includegraphics[width=\linewidth]{./images/dimenet/all.pdf}
    \caption{DimeNet$++$ architecture. Left to right: general structure, \emph{Embedding} block, \emph{Output} block. }
    \label{fig:dimenet}
\end{figure}

\begin{figure}[!t]\centering
    \includegraphics[width=.8\linewidth]{./images/dimenet/interaction.pdf}
    \caption{DimeNet$++$ architecture: the \emph{Interaction} block. }
    \label{fig:dimenet_interaction}
\end{figure}

\emph{DimeNet} is inspired by the \emph{PhysNet} model~\cite{unke2019physnet} and expands it with message passing and additional directional information. A general overview of the architecture is shown in Figure~\ref{fig:dimenet} (left).
The core of \emph{DimeNet} is the \emph{Interaction} block: a message $\mathbf{m}_{ji}$ from atom $j$ to atom $i$ takes into account information about the angles $\angle \mathbf{x}_i\mathbf{x}_j\mathbf{x}_k$ obtained via messages from the corresponding atoms $k$ that are neighbors of atom $j$. Specifically, it is defined as follows:
$$
\mathbf{m}_{ji}^{(l+1)} =
f_\textrm{update}\left(
\mathbf{m}_{ji}^{(l)},
\sum_{k\in\mathcal{N}_j\backslash\{i\}}
f_\textrm{int}\left(\mathbf{m}_{kj}^{(l)}, \mathbf{e}_\textrm{RBF}^{(ji)}, \mathbf{a}_\textrm{SBF}^{(kj,ji)}\right)
\right),
$$
where $\mathcal{N}_j$ is the set of neighbors of atom $j$, $\mathbf{e}_\textrm{RBF}^{(ji)}$ is the radial basis interatomic distance, and $\mathbf{a}_\textrm{SBF}^{(kj,ji)}$ is the directional information represented by spherical Bessel functions and spherical harmonics. 

The \emph{Interaction} block is visualized in Figure~\ref{fig:dimenet_interaction}. A message $\mathbf{m}_{ji}$ is initialized with learnable embeddings $\mathbf{h_i^{(0)}}$ and $\mathbf{h_j^{(0)}}$ that depend on the relative position of corresponding atoms (Fig.~\ref{fig:dimenet}, middle). Finally, the messages are combined together to form the atom embedding 
$$\mathbf{h}_i = \sum_{j\in\mathcal{N}_i}\mathbf{m}_{ji},$$ which is further used to predict the energy (Fig.~\ref{fig:dimenet}, right).

The resulting model is invariant to permutations, translation, rotation, and inversion. Evaluation on QM9 and MD17 shows that \emph{DimeNet} significantly outperforms \emph{SchNet} on the prediction of most targets. An extension of this model was later proposed in \emph{DimeNet++} ~\cite{gasteiger2020dimenetpp}; it further improved performance and reduced computational costs.

\ber{
\subsection{Graphormer}
\emph{Graphormer} is a Transformer-based architecture for graph related tasks presented in \citet{graphormer}. To adapt Transformer architecture for graph-based data, authors proposed 3 ways to encode data: centrality encoding, spatial encoding, and edge encoding.}
\ber{
Centrality encoding uses degree centrality to highlight the importance of a node in the graph: to each node of the graph, it assigns two embedding vectors according to the node's indegree and outdegree, subsequently summed with node features:
$$h_i^{0} = x_i + z^{-}_{deg^{-}(v_i)} + z^{+}_{deg^{+}(v_i)}$$
Spatial information is encoded with the shortest path between nodes $v_i$ and $v_j$ if they're connected, otherwise it's set to -1. Spatial encoding serves as a bias term in the self-attention module. For an edge encoding, it averages  dot-products between edge features and embeddings for one of shortest path $SP_{ij} = (e_1, e_2, ..., e_N)$ between nodes $v_i$ and $v_j$. Both encodings serve as bias terms for an attention module. Consider $A_{ij}$ is a (i,j)-element of the Query-Key product matrix
$$A_ij = \frac{(h_iW_Q)(h_jW_K)^T}{\sqrt{d}} + b_{\phi(v_i, v_j)} + c_{ij}, \; c_{ij} = \frac{1}{N}\sum^{N}_{n=1}x_{e_n}(\omega^{E}_n)^T,$$
$b_{\phi(v_i, v_j)}$ is a learnable scalar of spatial encoding shared across all attention heads, $x_{e_n}$ is an edge features from the n-th edge in $SP_{ij}$, $\omega^{E}_n$ - n-th weight embedding.\\
\emph{Graphormer3D} is an adaptation of \emph{Graphormer} for 3D molecular modelling tasks described in \cite{graphormer3D}. For spatial encoding, the set of Gaussian basis functions on Euclidean distances between nodes $v_i$ and $v_j$  was used. The centrality encoding is a sum of spatial encodings for each node in the graph. For node-level properties prediction, modified attention module takes output from standard self-attention module and decomposed it into three directions multiplying by relative position $\frac{r_{ij}}{||r_{ij}||}$, further three linear projection heads applied to each component.\\
}

\ber{
\subsection{GemNet}
A geometric message passing neural network (GemNet) is proposed in \citet{gemnet} and represents the development of ideas from DimeNet++. Additionally to one-hop message passing from DimeNet, GemNet uses a two-hop message passing mechanism. All atom pairs are embedded within cutoff distance and directional embedding updated considering quadruplets of atoms, where two atoms are interacting and two atoms define direction. Consider update for atom pair $c$ and $a$, set of atoms interacts with $a$ $\mathcal{N}_{int}^{a}$ with cutoff $c_{int}$ and set of neighbour atoms to $b$ $\mathcal{N}_{emb}^{b}$ with cutoff $c_{emb}$:
$$m_{ca} = \sum\limits_{\substack{b \in \mathcal{N}_{int}^{a} \backslash \{c\},\\ d \in \mathcal{N}_{emb}^{b} \backslash \{a, c\}}}((W_{SBF}e_{SBF}(x_{ca}, \phi_{cab}, \theta_{cabd}))^T\bold{W}((W_{CBF}e_{CBF}(x_{ba}, \phi_{abd})\odot(W_{RBF}e_{RBF}(x_{db}) \odot m_{db}))$$
where $W$ is weight matrix, $\mathbf{W}$ - weight tensor and $\theta_{cabd}$ is dihedral angle between two atom pairs. Two-hop means that the model incorporates messages from neighbor atom pairs into message update. Embeddings also update symmetrical, e.g., update influences both $m_{ca}$ and $m_{ac}$, preserving $m_{ca} \ne m_{ac}$ using two separate weight matrices. Then, results from interaction blocks are summed up and used for prediction energies and atomic forces.}

\ber{
GemNet-OC described in \citet{gemnet-oc} proposes modernized GemNet architecture. Instead of the fixed cutoff model uses the maximum number of neighbors because a fixed cutoff could lead to poor performance in the case of atom systems, where atoms are farther apart than 6\AA. Atom quadruplets interaction radius decreased based on empirical observations. Atom embeddings are now directly involved in the message passing scheme with atom-to-edge, edge-to-atom, and atom-to-atom interactions. This leads to hierarchy of different interactions, where costly atom quadruplets interactions used on short distance, interactions between edges are used on medium distance and atom-to-atom interactions could be used on long distances above due to their low computational complexity. These improvements lead to training time decreases and better results.
}

\subsection{SchNOrb \texorpdfstring{\citep{schnorb2019}}{}} This model is a direct continuation of the \emph{SchNet} model~\cite{schnet2017}; the \emph{SchNet} sub-architecture is used as a ``first step'' in the \emph{SchNOrb} model. The most important differences are the following:
\begin{inparaenum}[(1)]
\item \emph{SchNOrb} is designed to predict molecular energy, forces, the overlap matrix, and the Hamiltonian matrix;
\item directions (angles and normalized position differences) are used explicitly to capture the interaction information and model various symmetries;
\item the loss function is a sum of errors in the prediction of energy, forces, Hamiltonian, and the overlap matrix.
\end{inparaenum}

\begin{figure}[!t]
    \includegraphics[width=\linewidth]{./images/schnorb/all.pdf}
    \caption{The \emph{SchNOrb} architecture. On the left: general architecture overview; on the right: the \emph{Interaction} block in \emph{SchNOrb}. In addition to the \emph{SchNet} \emph{Interaction} block, \emph{SchNOrb} uses the factorized tensor layer\cite{schutt2017quantum} to produce pairwise atom features and predict the basis coefficients for the Hamiltonian.}
    \label{fig:schnorb}
\end{figure}

The inputs for this neural network are the charges $Z$ and position differences $\|\mathbf{r}_{ij}\|$ (norm of the vector pointing from atom $i$ to atom $j$); the model also uses normalized directions $\frac{\mathbf{r}_{ij}}{\|\mathbf{r}_{ij}\|}$.
The representations $Z$ and $\{\|\mathbf{r}_{ij}\|\}$ are then processed with the \emph{SchNet} step as described in Section~\ref{ssec:schnet}.

On the next \emph{SchNOrb} step, \emph{SchNet} outputs (a vector per atom) are combined with $\{\|\mathbf{r}_{ij}\|\}$ using a factorised tensor layer~\cite{schutt2017quantum}, feedforward layers, shifted softplus, and simple sums. The outputs include:
\begin{inparaenum}[(1)] 
\item rotationally invariant per-atom embeddings $\mathbf{X}^l$, which are then transformed and aggregated to predict the energy value;
\item embeddings $P^l$ for atom pairs that are multiplied by different powers of directional cosines, aggregated and passed to fully connected layers to predict blocks of the Hamiltonian and overlap matrices; 
\item finally, similar to \emph{SchNet}, forces are predicted via graph differentiation.
\end{inparaenum}
%%% data


The datasets used in this work are based on MD17~\cite{chmiela2017machine} and include water, ethanol, malondialdehyde, and uracil. Reference calculations were performed with Hartree-Fock (HF)
and density functional theory (DFT) with the PBE exchange correlation functional. For more details regarding data preparation and augmentation, we refer to~\citet{schnorb2019}.

% We train separate
% neural networks for several data sets of water as well as ethanol,
% malondialdehyde, and uracil from the MD17 dataset 7 . The
% reference calculations were performed with Hartree-Fock (HF)
% and density functional theory (DFT) with the PBE exchange
% correlation functional34 . The employed Gaussian atomic orbital
% bases include angular momenta up to l = 2 (d-orbitals). We
% augment the training data by adding rotated geometries and
% correspondingly rotated Hamiltonian and overlap matrices to
% learn the correct rotational symmetries (see Methods section).
% Detailed model and training settings for each data set are listed in
% Supplementary Table 1.


\input{table.tex}


\subsection{SE3 (PhiSNet)}\label{subsection:phisnet}
The \emph{PhiSNet} model was suggested by \citet{phisnet2021}. The authors presented an SE(3)-equivariant architecture for predicting Hamiltonian matrices. The model improves over the results of \emph{SchNOrb} both in terms of equivariance (\emph{SchNOrb} is not SE(3)-equivariant, so its predictions for the same conformation in a different reference coordinate system may differ in unpredictable ways) and in terms of accuracy metrics for single compound datasets.

\begin{figure}[!t]
    \includegraphics[width=\linewidth]{./images/phisnet/all.pdf}
    \caption{\emph{PhiSNet} architecture. On the left: general architecture overview; on the right: the \emph{PModule} block in detail. More details about sphilinear and interaction blocks of \emph{PModule} are given in \citet{phisnet2021}.}
    \label{fig:phisnet}
\end{figure}

The main building blocks of \emph{PhiSNet} are the following:
\begin{inparaenum}[(1)]
\item feature representation both for input and intermediate layers is of the form $\mathbb{R}^{F \times (L+1)^2}$, where $F$ corresponds to feature channels and $(L+1)^2$ corresponds to all possible spherical harmonics of degree $l \in \{0,\dots, L\}$;
\item all layers except the last one apply SE(3)-equivariant operations on features; matrix multiplication, tensor product contractions, and tensor product expansions are mixed together to make equivariant updates for the features of every atom and atom pair;
\item on the last layer, the Hamiltonian and overlap matrices are constructed from pairwise features.
\end{inparaenum}

We have made several minor modifications to the original model implementation of \emph{PhiSNet} in order to allow it to work with the \emph{$\nabla^2$DFT} dataset; in particular,
we have applied batchization similar to \emph{Pytorch Geometric}, where molecules inside a single batch are treated as one molecule with no bonds between atoms of different molecules.

\subsection{eSCN}\label{subsection:eSCN}
\emph{eSCN} is an improvement of \emph{SCN}(\cite{zitnick2022spherical}) described in \cite{SaroESCN}. Like PhiSNet \ref{subsection:phisnet}, \emph{SCN}-network uses the set of spherical harmonics as the atomical embeddings and tensor product operations to mix the features of different atoms. The messages and interactions are computed with the following  formulas:
\begin{equation}
\bm{m}_{st}^{(k+1)}(\bm{x}^{(k)}_s, \bm{x}^{(k)}_t, \bm{d}_{st}, a_s, a_t) = \mathbf{D}_{st}^{-1} \bm{F}_e (\mathbf{D}_{st} \bm{x}^{(k)}_s, \mathbf{D}_{st} \bm{x}^{(k)}_t, |\bm{d}_{st}|, a_s, a_t),
\label{eqn:msg}
\end{equation}

\begin{equation}
{\bm{x}}_t^{(k+1)} = \bm{x}_t^{(k)} + \bm{G}^{-1}\left(\bm{F}_c\left(\bm{G}(\bm{m}_{t}^{(k+1)}), \bm{G}(\bm{x}_t^{(k)})\right)\right),
\label{eqn:aggr}
\end{equation}
Here, $\mathbf{D}^l_{st}$ corresponds to the collections of Wigner D-matrices $\mathbf{D}^l$ of size $(2l+1 \times 2l+1)$ that rotates the coefficients of degree $l$ by the rotation $\mathbf{R}$, which rotates the $d_{st}$ (vector from atom $s$ to atom $t$) to the $z$-axis, $F_e$ is a GNN-layer, and, finally, $G$ is a function that converts a spherical function represented by spherical harmonic coefficients, to one represented by point samples on a sphere and $\bm{F}_{c}$ is a $1 \times 1$ convolutional neural network, which combines information across feature channels.

Finally, the energy and forces are predicted as:
\begin{equation}
E = \sum_i \int \bm{F}_{energy}\left(s_{i}^{(K)}(\hat{\bm{r}})\right)d\hat{\bm{r}},
\label{eqn:energy}
\end{equation}
and
\begin{equation}
\bm{f}_i = \int \hat{\bm{r}}\bm{F}_{force}\left(s_{i}^{(K)}(\hat{\bm{r}})\right)d\hat{\bm{r}},
\label{eqn:force}
\end{equation}


where $s_i$ is an output embedding corresponding to an $i$-th atom and $\bm{F}_{energy}$, $\bm{F}_{forces}$ are fully connected networks. Moreover, $f_i$ may be computed directly like in PaiNN~\ref{ssec:painn} via graph differentiation, but in this work, we experiment only with additional network variants.

Finally, \emph{eSCN} improves \emph{SCN} architecture with $SO(2)$-convolutions, which replace $SO(3)$-convolutions. This replacement improves both the network's computational efficiency and  the quality in terms of the loss functions.

\subsection{EquiformerV2}

\emph{EquiformerV2} is an improvement of \emph{Equiformer}~\cite{liao2022equiformer} architecture described in \cite{liao2023equiformerv2}.
In \emph{Equiformer}, the atomical representation, like in PhiSNet~\ref{subsection:phisnet} and \emph{eSCN}~\ref{subsection:eSCN}, is based on spherical harmonics, while the interactions layers additionally use Equivariant Graph Attention.

During the interaction, first, atom embeddings are merged with the Depth-wise Tensor Product (\emph{DTP}) layer, the attention coefficients are computed from the 0-order component, and finally, higher-order features are updated with attention coefficients by the tensor product operation and passed into a linear layer, see \ref{fig:equiformer}.

\begin{figure}[!t]
    \includegraphics[width=\linewidth]{./images/equiformer/Equiformer.pdf}
    \caption{\emph{Equiformer} architecture. On the left: general architecture overview; in the middle: Equivariant transformer encoder module (ETE) overview; on the right: the schematic architecture of the equivariant attention layer (EAtt)}
    \label{fig:equiformer}
\end{figure}

Finally, \emph{EquiformerV2} improves \emph{Equiformer} architecture with $SO(2)$-convolutions, which replace \emph{DTP} layer,  attention re-normalization, separable $S^2$ activation, and separable layer normalization, which replaces Layer Norm.



==> XX_supplementary_materials.tex <==




%\begin{landscape}
\begin{table}[]
\caption{Summary of quantum chemistry dataset. (+) denotes information that is not provided in a direct way in article or descriptions. (*) denotes parameters that can be derived from dataset with some computation.}\label{tbl:dataset-summary}
\tiny
\addtolength{\tabcolsep}{-1pt} 
\begin{tabular}{llllllllll} \hline
                                                                   & \textbf{NablaDFT2}                                                               & \textbf{NablaDFT}                                                                  & \textbf{QM7}                                                                                & \textbf{QM7b}                                                                                   & \textbf{QM7-X}                                                                          & \textbf{QM9}                                                                            & \textbf{\begin{tabular}[c]{@{}l@{}}MultiXC-\\ QM9\end{tabular}}                          & \textbf{QM1B}                                                          & \textbf{QH9}                                                                                      \\ \hline
\begin{tabular}[c]{@{}l@{}}Chem. inf.\\ Source\end{tabular}        & \begin{tabular}[c]{@{}l@{}}MOSES,\\ ZINC21\\ (Zinc\\ Clean\\ Leads)\end{tabular} & \begin{tabular}[c]{@{}l@{}}MOSES,\\ ZINC21\\ (Zinc \\ Clean \\ Leads)\end{tabular} & GDB-13                                                                                      & GDB-13                                                                                          & GDB-13                                                                                  & GDB-17                                                                                  & GDB-17                                                                                   & GDB-11                                                                 & \begin{tabular}[c]{@{}l@{}}GDB-13, \\ QM9\end{tabular}                                            \\
\begin{tabular}[c]{@{}l@{}}\# of\\ molecules\end{tabular}          & 2M                                                                               & 1M                                                                                 & 7K                                                                                          & 7K                                                                                              & 7K                                                                                      & 134K                                                                                    & 134K                                                                                     & 1M                                                                     & 130K                                                                                              \\
\begin{tabular}[c]{@{}l@{}}\# of \\ conformers\end{tabular}        & 13M                                                                              & 5M                                                                                 & 7K                                                                                          & 7K                                                                                              & 4M                                                                                      & 134K                                                                                    & 134K                                                                                     & 1B                                                                     & 130K                                                                                              \\
\begin{tabular}[c]{@{}l@{}}\# of \\ atoms\end{tabular}             & 8-62                                                                             & 8–62                                                                               & 1-23                                                                                        & 1-23                                                                                            & 1-23                                                                                    & 3-29                                                                                    & 3-29                                                                                     & 9-11                                                                   & 3-29                                                                                              \\
\begin{tabular}[c]{@{}l@{}}\# of \\ heavy \\ atoms\end{tabular}    & 8-27                                                                             & 8–27                                                                               & 1-7                                                                                         & 1-7                                                                                             & 1-7                                                                                     & 1-9                                                                                     & 1-9                                                                                      & +                                                                      & 1-9\\
Atoms                                                              & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O,S, Cl,\\ F,Br\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O,Cl,F,\\ Br\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O,S\end{tabular}                                        & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O,S\end{tabular}                                            & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O,S,Cl\end{tabular}                                 & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O,F\end{tabular}                                    & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O,F\end{tabular}                                     & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O,F\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O,F\end{tabular}                                              \\
\begin{tabular}[c]{@{}l@{}}Forces\end{tabular}             & Yes                                                                              & Yes                                                                                & No                                                                                          & No                                                                                              & Yes                                                                                     & No                                                                                      & No                                                                                       & No                                                                     & Yes                                                                                               \\
\begin{tabular}[c]{@{}l@{}}Hamilt-\\onians\end{tabular}                                                   & Yes                                                                              & Yes                                                                                & No                                                                                          & No                                                                                              & No                                                                                      & No                                                                                      & No                                                                                       & No                                                                     & No                                                                                                \\
\begin{tabular}[c]{@{}l@{}}Optim\\ traj.\end{tabular}              & Yes                                                                              & No                                                                                 & No                                                                                          & No                                                                                              & No                                                                                      & No                                                                                      & No                                                                                       & No                                                                     & Yes                                                                                               \\
\begin{tabular}[c]{@{}l@{}}Basis set\\ and\\ XC-func.\end{tabular} & \begin{tabular}[c]{@{}l@{}}$\Omega$B97X-\\ D/\\ Def2-\\ SVP\end{tabular}         & \begin{tabular}[c]{@{}l@{}}$\Omega$B97X-\\ D/\\ Def2-\\ SVP\end{tabular}           & PBE0                                                                                        & \begin{tabular}[c]{@{}l@{}}ZINDO, \\ SCS, \\ PBE0, \\ GW\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}ePBE0+\\ MBD, \\ TotFOR\end{tabular}                         & \begin{tabular}[c]{@{}l@{}}B3LYP/6-\\ 31G(2df,p)\\ + G4MP2\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}B3LYP and PBE/\\ 6–31G(2df,p),\\ SZ, DZP,\\ TZP\end{tabular} & \begin{tabular}[c]{@{}l@{}}STO-3G/\\ B3LYP\end{tabular}                & \begin{tabular}[c]{@{}l@{}}B3LYP/\\ Def2SVP\end{tabular}                                          \\
\begin{tabular}[c]{@{}l@{}}Storage\\ size\end{tabular}             & 220 Tb                                                                           & 100 Tb                                                                             & 17.9 MB                                                                                     & 16.1 MB                                                                                         & 1.35 Gb                                                                                 & 230 Mb                                                                                  & 317 Gb                                                                                   & 240 GB                                                                 & 28.4 Gb                                                                                           \\ \hline
                                                                   & \textbf{GEOM}                                                                    & \textbf{ANI-1}                                                                     & \textbf{\begin{tabular}[c]{@{}l@{}}ANI-1x/\\ ANI-1cxx\end{tabular}}                         & \textbf{\begin{tabular}[c]{@{}l@{}}OrbNet\\ Denali\end{tabular}}                                & \textbf{QMugs}                                                                          & \textbf{SPICE}                                                                          & \textbf{PubChemQC}                                                                       & \textbf{Frag20}                                                        & \textbf{VQM24}                                                                                    \\ \hline
\begin{tabular}[c]{@{}l@{}}Chem. inf.\\ Source\end{tabular}        & \begin{tabular}[c]{@{}l@{}}QM9,\\ AICures\end{tabular}                           & GDB                                                                                & \begin{tabular}[c]{@{}l@{}}GDB-11,\\ ChEMBL\end{tabular}                                    & ChEMBL27                                                                                        & ChEMBL                                                                                  & \begin{tabular}[c]{@{}l@{}}PubChem+\\ DES370K+\\ Other\end{tabular}                     & PubChem                                                                                  & \begin{tabular}[c]{@{}l@{}}PubChem,\\ ZINC\end{tabular}                & \textit{\begin{tabular}[c]{@{}l@{}}Combi- \\ natorial\end{tabular}}                               \\
\begin{tabular}[c]{@{}l@{}}\# of\\ molecules\end{tabular}          & 450K                                                                             & 57K                                                                                & 57K                                                                                         & 16K                                                                                             & 665K                                                                                    & 19K                                                                                     & 85M                                                                                      & 565K                                                                   & 10K                                                                                               \\
\begin{tabular}[c]{@{}l@{}}\# of \\ conformers\end{tabular}        & 37M                                                                              & 24M                                                                                & 20M                                                                                         & 2.3M                                                                                            & 2M                                                                                      & 1KK                                                                                     & 85M                                                                                      & 566K                                                                   & 835K                                                                                              \\
\begin{tabular}[c]{@{}l@{}}\# of \\ atoms\end{tabular}             & +                                                                                & +                                                                                  & 2-26                                                                                        & +                                                                                               & 4-228                                                                                   & 2–96                                                                                    & +                                                                                        & +                                                                      & 4,5                                                                                               \\
\begin{tabular}[c]{@{}l@{}}\# of \\ heavy \\ atoms\end{tabular}    & +                                                                                & 1-11                                                                               & 1-8                                                                                         & +                                                                                               & 4-100                                                                                   & +                                                                                       & 51                                                                                       & 20                                                                     & +                                                                                                 \\
Atoms                                                              & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O,F,+\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O\end{tabular}                                 & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O\end{tabular}                                          & \begin{tabular}[c]{@{}l@{}}H,Li,B,\\ C,N,O,\\ F,Na,Mg,\\ Si,P,S,\\ Cl,K,Ca,\\ Br,I\end{tabular} & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O,P,S,\\ Cl,F,Br,\\ I\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}H,Li,C,\\ N,O,F,\\ Na,Mg,P,\\ S,Cl,K,\\ Ca,Br,I\end{tabular} & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O,P,S, \\ F,Cl,Na\\ K,Mg,Ca,\end{tabular}            & \begin{tabular}[c]{@{}l@{}}H,B,C,\\ O,N,F,\\ P,S,Cl,\\ Br\end{tabular} & \begin{tabular}[c]{@{}l@{}}H,C,N,\\ O,F,Si,\\ P,S,Cl,\\ Br\end{tabular}                           \\
\begin{tabular}[c]{@{}l@{}}Forces\end{tabular}             & Yes                                                                              & No                                                                                 & No                                                                                          & No                                                                                              & No*                                                                                     & Yes                                                                                     & No                                                                                       & No                                                                     & No                                                                                                \\
\begin{tabular}[c]{@{}l@{}}Hamilt-\\onians\end{tabular}         & No                                                                               & No                                                                                 & No                                                                                          & No                                                                                              & No*                                                                                     & No                                                                                      & No                                                                                       & No                                                                     & No                                                                                                \\
\begin{tabular}[c]{@{}l@{}}Optim\\ traj.\end{tabular}              & No                                                                               & No                                                                                 & No                                                                                          & No                                                                                              & No                                                                                      & No                                                                                      & No                                                                                       & No                                                                     & No                                                                                                \\
\begin{tabular}[c]{@{}l@{}}Basis set\\ and\\ XC-func.\end{tabular} & \begin{tabular}[c]{@{}l@{}}mTZVPP/\\ R2scan-3\end{tabular}                       & \begin{tabular}[c]{@{}l@{}}WB97x/\\ 6–31g(d)\end{tabular}                          & \begin{tabular}[c]{@{}l@{}}wB97x/\\6-31G*, \\ wB97x/\\def2-TZVPP, \\ CCSD(T)*/\\CBS,\end{tabular} & \begin{tabular}[c]{@{}l@{}}$\Omega$B97X-\\ D3/\\ Def2-\\ TZVP\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}$\omega$B97X-\\ D/\\ Def2-\\ SVP\\ +GFN2-\\ XTB\end{tabular} & \begin{tabular}[c]{@{}l@{}}$\omega$B97M-\\ D3(BJ)/\\ Def2-\\ TZVPPD\end{tabular}        & \begin{tabular}[c]{@{}l@{}}B3LYP/\\ 6-31G*+\\ PM6\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}B3LYP/\\ 6-31G*\end{tabular}                & \begin{tabular}[c]{@{}l@{}}$\Omega$B97X-D3/\\ Cc-\\ pVDZ,\\ DMC@\\PBE0(cEC/\\ Cc-VQZ))\end{tabular} \\
\begin{tabular}[c]{@{}l@{}}Storage\\ size\end{tabular}             & 130.8 GB                                                                         & 4.48 Gb                                                                            & 5.29 Gb                                                                                     & 2.74 GB                                                                                         & 7 Tb                                                                                    & 37.5 GB                                                                                 & 100 Tb                                                                                   & 566 Mb                                                                 & 1.5 Gb                                                                                  \\\hline    
\end{tabular}
\addtolength{\tabcolsep}{1pt} 
\end{table}

%\end{landscape}



\begin{table}[]
  \caption{Properties available for each data instance in $\nabla^2$DFT.}\label{tbl:properties}
  \footnotesize
\begin{tabular}{cl}
\hline
\multicolumn{1}{c}{Access mode}                                              & \multicolumn{1}{c}{Content}                                       \\ \hline
\begin{tabular}[c]{@{}l@{}}Main data\\ (from basic\\dataloader)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Atoms numbers, atoms positions, energy ('DFT FORMATION ENERGY'), forces, \\  Hamiltonian (Fock matrix), overlap matrix, coefficients matrix\end{tabular}\\  \hline 
\begin{tabular}[c]{@{}c@{}}Metainformation\\ (from\\summary.csv)\end{tabular} & \begin{tabular}[c]{@{}l@{}}'DFT TOTAL ENERGY', 'DFT XC ENERGY', 'DFT NUCLEAR REPULSION ENERGY', \\ 'DFT ONE-ELECTRON ENERGY', 'DFT TWO-ELECTRON ENERGY', \\ 'DFT DIPOLE X', 'DFT DIPOLE Y', 'DFT DIPOLE Z', 'DFT TOTAL DIPOLE',\\ 'DFT ROT CONSTANT A', 'DFT ROT CONSTANT B', 'DFT ROT CONSTANT C',\\ 'DFT HOMO', 'DFT LUMO', 'DFT HOMO-LUMO GAP', \\ 'DFT ATOMIC ENERGY', 'DFT FORMATION ENERGY'\end{tabular}                                                                               \\  \hline
\begin{tabular}[c]{@{}c@{}}Raw stored\\ wavefunction\\ object\end{tabular}   & \begin{tabular}[c]{@{}l@{}}All DATA FROM TWO PREVIOUS ROWS, \\ Ca/Cb (molecular orbital coefficients), Da/Db (density matrix), Fa/Fb (Fock matrix), \\ H (Core Hamiltonian), S (overlap matrix), X (XC-functional matrix), \\ aotoso (Atomic Orbital to Symmetry Orbital), epsilon\_a/epsilon\_b (orbital eigenvalues), \\ SCF DIPOLE, doccpi (number of doubly occupied orbitals), nmo (number of molecule orbitals),\\ 'DISPERSION CORRECTION ENERGY', 'GRID ELECTRONS TOTAL'\end{tabular} \\  \hline
\begin{tabular}[c]{@{}l@{}}Available after \\ loading into Psi4\end{tabular} & \begin{tabular}[c]{@{}l@{}}All DATA FROM THREE PREVIOUS ROWS, \\ Electric dipole moment, Electric quadrupole moment, All moments up order N, \\ Electrostatic potential at nuclei, Electrostatic potential on grid, Electric field on grid, \\ Molecular orbital extents, Mulliken atomic charges, Löwdin atomic charges, \\ Wiberg bond indices, Mayer bond indices, Natural orbital occupations, \\ Stockholder Atomic Multipoles, Hirshfeld volume ratios\end{tabular}                    \\ \hline
\end{tabular}
\end{table}























\iffalse

\begin{table*}
  \caption{DFT dataset statistics}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}|c|p{2cm}|p{2cm}|p{2cm}|p{2cm}|}
    \hline
    \textbf{Statistic} & \textbf{QM9} & \textbf{ANI-1} & \textbf{QMugs} & \textbf{$\nabla^2$DFT}\\
    \hline
    Number of molecules & $134$K & \numprint{57462} & $665$K & $2$M\\
    Number of conformers &   $134$K  & $20$M & $2$M  & $13$M\\
    Number of atoms & $3$-$29$ & $2$-$26$ & $4$-$228$ &  $8$-$62$\\
    Number of heavy atoms & $1$-$9$ & $1$-$8$ & $4$-$100$ & $8$-$27$ \\
    Atomic species & H, C, N, O, F &  H, C, N, O & H, C, N, O, P, S, Cl, F, Br, I &  H, C, N, O, S, Cl, F, Br\\
    Forces matrices &No & No& No$^{*}$&  Yes\\
    Optimization trajectories &No & No& No&  Yes\\
    
    Hamiltonian matrices &No & No& No$^{*}$&  Yes\\
    Level of theory & \small  B3LYP/6-31G(2df,p) \newline + G4MP2  & \small $\omega$B97X/\newline6–31G(d) & \small $\omega$B97X-D/def2-SVP \newline + \small GFN2-xTB &$\omega$B97X-D/def2-SVP \\
    Storage Size&   230 Mb  & 5.29 Gb & 7 Tb & 220 Tb\\
    \hline
  \end{tabular*}
  \label{tbl:dft_datasets}
  \small{\textit{*} Hamiltonian matrices for QMugs dataset can be calculated from density matrices by one step of DFT cycle}
\end{table*}


\begin{table*}
  \caption{Properties provided in DFT datasets}
  \begin{tabular*}{\textwidth}{| c   | @{\extracolsep{\fill}} p{12cm}|}
    \hline
    \textbf{QM9} & 
    DFT + partially G4MP2: Rotational constants, dipole moment, isotropic polarizability, HOMO/LUMO/gap energies, electronic spatial extent, zero point vibrational energy, internal energy at 0 K, internal energy at 298.15 K, enthalpy at 298.15 K, free energy at 298.15 K, heat capacity at 298.15 K, Mulliken charges, harmonic vibrational frequencies
    \\
    \hline
    \textbf{ANI-1} & 
    DFT:Total energy
    \\
    \hline
    \textbf{QMugs} &
    GFN2+DFT: Total, internal atomic and formation energies, Dipole, Rotational constants, HOMO/LUMO/gap energies, Mulliken partial charges \newline
    GFN2: Total enthalpy, Total free energy, Quadrupole, Enthalpy, Heat capacity, Entropy, Fermi level, Covalent coordination number, Molecular dispersion coefficient, Atomic dispersion coefficients, Molecular polarizability, Atomic polarizabilities, Wiberg bond orders, Total Wiberg bond orders \newline
    DFT: Electrostatic potential, Löwdin partial charges, Exchange correlation energy, Nuclear repulsion energy, One-electron energy, Two-electron energy, Mayer bond orders, Wiberg-Löwdin bond orders, Total Mayer bond orders, Total Wiberg-Löwdin bond orders, Density/orbital matrices, atomic-orbital-to-symmetry-orbital transformer matrix
    \\
    \hline
    \textbf{$\nabla^2$DFT} &
    DFT: Electrostatic potential, Löwdin partial charges, Exchange correlation energy, Nuclear repulsion energy, One-electron energy, Two-electron energy, Mayer bond orders, Wiberg-Löwdin bond orders, Total Mayer bond orders, Total Wiberg-Löwdin bond orders, Density/orbital matrices, atomic-orbital-to-symmetry-orbital transformer matrix, Hamiltonian matrix, Atomic Forces
    \\
    \hline
  \end{tabular*}
  \label{tbl:dft_datasets_properties}
\end{table*}

\fi

==> table.tex <==
%\begin{table*}[!ht]
% \caption{Energy prediction metrics: mean absolute error (MAE), less is better.}
%  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}|l|P{.1\linewidth}|P{.1\linewidth}|P{.18\linewidth}|P{.1\linewidth}|}
%        \hline
%    \multirow{2}{*}{\textbf{Model}} &
%      \multicolumn{4}{c|}{\textbf{MAE for energy prediction}, $\times 10^{-2}  E_h$}\\
%    & $\mathcal{D^{\text{tiny}}}$ & $\mathcal{D^{\text{small}}}$ & $\mathcal{D^{\text{medium}}}$ & $\mathcal{D^{\text{large}}}$ \\
%      \hline 
%     \multicolumn{1}{|c}{}&\multicolumn{4}{c|}{\textbf{Structure test split}}\\
%    \hline
%    LR &  4.86 &  4.64 &  4.56 &  4.56 \\
      % \hline 
%    SchNet & 1.17 &  0.90 &  1.10 &  0.31 \\
%    PaiNN & \textbf{0.82} &  0.60 &  0.36 &  \textbf{0.09} \\
      % \hline
%    Dimenet++  & 42.84 &  0.56 &  \textbf{0.21} & \textbf{0.09} \\
     % \hline
%    SchNOrb & 0.83 &  \textbf{0.47} &  0.39 & 0.39 \\
    % \hline
%    Graphormer3D$_{Small}$ & 1.54 & 0.96 & 0.77 & 0.37 \\
    % \hline
%    GemNet-OC & 2.79 & 0.65 & 0.28 & 0.22 \\
    % \hline
%    EquiformerV2  & 2.81 & 1.13 & 0.28 & 0.19 \\
    % \hline
%    eSCN & 1.87 & 0.47 & 0.94 & 0.42 \\
    % \hline
%    \hline
%    \multicolumn{1}{|c}{}&\multicolumn{4}{c|}{\textbf{Scaffolds test split}}\\
%    \hline
%    LR &  4.37 &  4.18 &  4.12 & 4.15 \\
      % \hline 
%    SchNet & 1.19 &  0.92 &  1.11 & 0.31 \\
%    PaiNN & \textbf{0.86} &  0.61 &  0.36 &  0.09 \\
      % \hline
%    Dimenet++  & 37.41 &  0.41 & \textbf{0.19} & \textbf{0.08} \\
     % \hline
%    SchNOrb & \textbf{0.86} &  \textbf{0.46} &  0.37 & 0.39  \\
%    Graphormer3D$_{Small}$ & 1.58 & 0.94 & 0.75 & 0.36 \\
    % \hline
%    GemNet-OC & 2.59 & 0.59 & 0.27 & 0.23 \\
    
%    EquiformerV2 & 2.65 & 1.13 & 0.27 & 0.17 \\
    % \hline
%    eSCN & 1.87 & 0.47 & 0.92 & 0.42 \\
    % \hline
%    \hline
%    \multicolumn{1}{|c}{}&\multicolumn{4}{c|}{\textbf{Conformations test split}}\\
%    \hline
%    LR &  3.76 &  3.61 &  3.69 & 3.95 \\
      % \hline 
%    SchNet & 0.56 &  0.63 &  0.88 & 0.28 \\
%    PaiNN & 0.43 &  0.49 &  0.28 &  0.08 \\
      % \hline
%    Dimenet++  & 0.42 &  \textbf{0.10} &  \textbf{0.09} &  \textbf{0.07}\\
     % \hline
%    SchNOrb & \textbf{0.37} &  0.26 &  0.27 & 0.36 \\
%    Graphormer3D$_{Small}$ & 0.99 & 0.67 & 0.58 & 0.39 \\
    % \hline
%    GemNet-OC & 0.52 & 0.2 & 0.15 & 0.24 \\
    % \hline
%    EquiformerV2 & 0.45 & 0.23 & 0.24 & 0.16 \\
    % \hline
%    eSCN & 0.48 & 0.31 & 0.80 & 0.44 \\
    % \hline

%    \hline
%  \end{tabular*}
%  \label{tbl:results_energy}
  
 
% \caption{Forces prediction metrics: mean absolute error (MAE), less is better.}
%  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}|l|P{.1\linewidth}|P{.1\linewidth}|P{.1\linewidth}|P{.1\linewidth}|}
%        \hline
%    \multirow{2}{*}{\textbf{Model}} &
%      \multicolumn{4}{c|}{\textbf{MAE for forces prediction}, $\times 10^{-2}  \frac{E_h}{A}$}\\
%    & $\mathcal{D^{\text{tiny}}}$ & $\mathcal{D^{\text{small}}}$ & $\mathcal{D^{\text{medium}}}$ & $\mathcal{D^{\text{large}}}$ \\
%      \hline 
%     \multicolumn{1}{|c}{}&\multicolumn{4}{c|}{\textbf{Structure test split}}\\
%    \hline
%    SchNet & 0.44 & 0.37 & 0.41 & 0.16 \\
%    PaiNN & 0.37 & 0.26 & 0.17 & 0.06 \\
      % \hline
%    Dimenet++  & 1.31 & 0.20 & 0.13 & 0.065 \\
     % \hline
%    Graphormer3D$_{Small}$ & 1.11 & 0.67 & 0.54 & 0.26 \\
    % \hline
%    GemNet-OC & 0.14 & 0.07 & 0.05 & \textbf{0.02} \\
%    EquiformerV2 & 0.30 & 0.23 & 0.21 & 0.17 \\
    % \hline
%    eSCN & \textbf{0.10} & \textbf{0.051} & \textbf{0.04} & \textbf{0.02} \\
    % \hline
%    \hline
%    \multicolumn{1}{|c}{}&\multicolumn{4}{c|}{\textbf{Scaffolds test split}}\\
%    \hline
%    SchNet & 0.45 & 0.37 & 0.41 & 0.16 \\
%    PaiNN & 0.38 & 0.26 & 0.17 & 0.06 \\
      % \hline
%    Dimenet++  & 1.36 & 0.19 & 0.13 & 0.066 \\
     % \hline
%    Graphormer3D$_{Small}$ & 1.13 & 0.68 & 0.55 & 0.26 \\
    % \hline
%    GemNet-OC & 0.14 & 0.06 & 0.04 & \textbf{0.02} \\
%    EquiformerV2 & 0.31 & 0.23 & 0.21 & 0.17 \\
    % \hline
%    eSCN & \textbf{0.10} & \textbf{0.05} & \textbf{0.036} & \textbf{0.021} \\
%    \hline
%    \multicolumn{1}{|c}{}&\multicolumn{4}{c|}{\textbf{Conformations test split}}\\
%    \hline
%    SchNet & 0.32 &  0.3 &  0.37 & 0.14 \\
%    PaiNN & 0.23 &  0.22 &  0.14 &  0.05 \\
      % \hline
%    Dimenet++  & 0.26 &  0.12 &  0.10 &  0.06\\
     % \hline
  %  Graphormer3D$_{Small}$ & 0.82 & 0.54 & 0.45 & 0.23 \\
    % \hline
 %   GemNet-OC & \textbf{0.07} & \textbf{0.04} & \textbf{0.03} & \textbf{0.02} \\
%    EquiformerV2 & 0.16 & 0.15 & 0.16 & 0.13 \\
    % \hline
%    eSCN & \textbf{0.065} & \textbf{0.037} & \textbf{0.029} & \textbf{0.021} \\
    % \hline
%    \hline
%  \end{tabular*}
%  \label{tbl:results_forces}

% \end{table*}
%\end{table*}

 % {\renewcommand{\arraystretch}{2}












\begin{table}[!t]
\begin{minipage}[t]{.48\linewidth}\centering\small
\caption{Energy prediction metrics: mean absolute error (MAE), less is better.}\label{tbl:results_energy}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|cccc}
    \toprule
 \multirow{2}{*}{\textbf{Model}} &
      \multicolumn{4}{C{.5\linewidth}}{\textbf{MAE for energy prediction}, $\times 10^{-2}  E_h$}\\
    & $\mathcal{D^{\text{tiny}}}$ & $\mathcal{D^{\text{small}}}$ & $\mathcal{D^{\text{medium}}}$ & $\mathcal{D^{\text{large}}}$ \\
      \midrule 
     \multicolumn{1}{c}{}&\multicolumn{4}{c}{\textbf{Structure test split}}\\
    \midrule
    LR &  4.86 &  4.64 &  4.56 &  4.56 \\
      % \hline 
    SchNet & 1.17 &  0.90 &  1.10 &  0.31 \\
    PaiNN & \textbf{0.82} &  0.60 &  0.36 &  \textbf{0.09} \\
      % \hline
    Dimenet++  & 42.84 &  0.56 &  \textbf{0.21} & \textbf{0.09} \\
     % \hline
    SchNOrb & 0.83 &  \textbf{0.47} &  0.39 & 0.39 \\
    % \hline
    Graphormer3D & 1.54 & 0.96 & 0.77 & 0.37 \\
    % \hline
    GemNet-OC & 2.79 & 0.65 & 0.28 & 0.22 \\
    % \hline
    EquiformerV2  & 2.81 & 1.13 & 0.28 & 0.19 \\
    % \hline
    eSCN & 1.87 & \textbf{0.47} & 0.94 & 0.42 \\
    % \hline
    \midrule
    \multicolumn{1}{c}{}&\multicolumn{4}{c}{\textbf{Scaffolds test split}}\\
    \midrule
    LR &  4.37 &  4.18 &  4.12 & 4.15 \\
      % \hline 
    SchNet & 1.19 &  0.92 &  1.11 & 0.31 \\
    PaiNN & \textbf{0.86} &  0.61 &  0.36 &  0.09 \\
      % \hline
    Dimenet++  & 37.41 &  \textbf{0.41} & \textbf{0.19} & \textbf{0.08} \\
     % \hline
    SchNOrb & \textbf{0.86} &  0.46 &  0.37 & 0.39  \\
    Graphormer3D & 1.58 & 0.94 & 0.75 & 0.36 \\
    % \hline
    GemNet-OC & 2.59 & 0.59 & 0.27 & 0.23 \\
    
    EquiformerV2 & 2.65 & 1.13 & 0.27 & 0.17 \\
    % \hline
    eSCN & 1.87 & 0.47 & 0.92 & 0.42 \\
    % \hline
    \midrule
    \multicolumn{1}{c}{}&\multicolumn{4}{c}{\textbf{Conformations test split}}\\
    \midrule
    LR &  3.76 &  3.61 &  3.69 & 3.95 \\
      % \hline 
    SchNet & 0.56 &  0.63 &  0.88 & 0.28 \\
    PaiNN & 0.43 &  0.49 &  0.28 &  0.08 \\
      % \hline
    Dimenet++  & 0.42 &  \textbf{0.10} &  \textbf{0.09} &  \textbf{0.07}\\
     % \hline
    SchNOrb & \textbf{0.37} &  0.26 &  0.27 & 0.36 \\
    Graphormer3D$_{Small}$ & 0.99 & 0.67 & 0.58 & 0.39 \\
    % \hline
    GemNet-OC & 0.52 & 0.20 & 0.15 & 0.24 \\
    % \hline
    EquiformerV2 & 0.45 & 0.23 & 0.24 & 0.16 \\
    % \hline
    eSCN & 0.48 & 0.31 & 0.80 & 0.44 \\
    \bottomrule 
\end{tabular}\vspace{.2cm}
\end{minipage}~~~~\begin{minipage}[t]{.48\linewidth}\centering\small
\caption{Forces prediction metrics: mean absolute error (MAE), less is better.}\label{tbl:results_forces}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|cccc}
\toprule
\multirow{2}{*}{\textbf{Model}} &
      \multicolumn{4}{C{.5\linewidth}}{\textbf{MAE for forces prediction}, $\times 10^{-2}  E_h / \textup{\AA}$}\\
    & $\mathcal{D^{\text{tiny}}}$ & $\mathcal{D^{\text{small}}}$ & $\mathcal{D^{\text{medium}}}$ & $\mathcal{D^{\text{large}}}$ \\
      \toprule  
     \multicolumn{1}{c}{}&\multicolumn{4}{c}{\textbf{Structure test split}}\\
    \midrule 
    SchNet & 0.44 & 0.37 & 0.41 & 0.16 \\
    PaiNN & 0.37 & 0.26 & 0.17 & 0.06 \\
      % \hline
    Dimenet++  & 1.31 & 0.20 & 0.13 & 0.07 \\
     % \hline
    Graphormer3D & 1.11 & 0.67 & 0.54 & 0.26 \\
    % \hline
    GemNet-OC & 0.14 & 0.07 & 0.05 & \textbf{0.02} \\
    EquiformerV2 & 0.30 & 0.23 & 0.21 & 0.17 \\
    % \hline
    eSCN & \textbf{0.10} & \textbf{0.05} & \textbf{0.04} & \textbf{0.02} \\
    % \hline
    \midrule 
    \multicolumn{1}{c}{}&\multicolumn{4}{c}{\textbf{Scaffolds test split}}\\
    \midrule 
    SchNet & 0.45 & 0.37 & 0.41 & 0.16 \\
    PaiNN & 0.38 & 0.26 & 0.17 & 0.06 \\
      % \hline
    Dimenet++  & 1.36 & 0.19 & 0.13 & 0.07 \\
     % \hline
    Graphormer3D & 1.13 & 0.68 & 0.55 & 0.26 \\
    % \hline
    GemNet-OC & 0.14 & 0.06 & \textbf{0.04} & \textbf{0.02} \\
    EquiformerV2 & 0.31 & 0.23 & 0.21 & 0.17 \\
    % \hline
    eSCN & \textbf{0.10} & \textbf{0.05} & \textbf{0.04} & \textbf{0.02} \\
    \midrule 
    \multicolumn{1}{c}{}&\multicolumn{4}{c}{\textbf{Conformations test split}}\\
    \midrule 
    SchNet & 0.32 &  0.30 &  0.37 & 0.14 \\
    PaiNN & 0.23 &  0.22 &  0.14 &  0.05 \\
      % \hline
    Dimenet++  & 0.26 &  0.12 &  0.10 &  0.06\\
     % \hline
    Graphormer3D & 0.82 & 0.54 & 0.45 & 0.23 \\
    % \hline
    GemNet-OC & \textbf{0.07} & \textbf{0.04} & \textbf{0.03} & \textbf{0.02} \\
    EquiformerV2 & 0.16 & 0.15 & 0.16 & 0.13 \\
    % \hline
    eSCN & \textbf{0.07} & \textbf{0.04} & \textbf{0.03} & \textbf{0.02} \\
\bottomrule 
\end{tabular}\vspace{.3cm}
\end{minipage}
\end{table}
\vspace*{-50px}

%\begin{table*}[!t]
%\caption{The $\overline{\operatorname{pct}_T}$ and $\operatorname{pct}_{\text{success}}$ for the geometry optimization task}
%\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}|l|P{.07\linewidth}|P{.07\linewidth}|P{.07\linewidth}|P{.07\linewidth}|P{.07\linewidth}|P{.07\linewidth}|P{.07\linewidth}|P{.07\linewidth}|}
%    \hline

%    \multirow{2}{*}{\textbf{Model}} &
%      \multicolumn{4}{c|}{$\displaystyle \overline{\operatorname{pct}}_T(\%)\uparrow$} &
%      \multicolumn{4}{c|}{$\operatorname{pct}_{\text{success}}(\%) \uparrow$ }\\
%    &$\mathcal{D^{\text{tiny}}}$ & $\mathcal{D^{\text{small}}}$ & $\mathcal{D^{\text{medium}}}$ & $\mathcal{D^{\text{large}}}$ & $\mathcal{D^{\text{tiny}}}$ & $\mathcal{D^{\text{small}}}$ & $\mathcal{D^{\text{medium}}}$ & $\mathcal{D^{\text{large}}}$\\
%      \hline 
%    SchNet & 61.35 & 65.00 & 61.10 & 80.82 & 0 & 0 & 0 & 1.15   \\
    % \hline
%    PaiNN & 69.31 & 73.66 & 76.99 & 89.40 & 0 & 0.15 & 1.00 & \textbf{11.05}   \\
    %DimeNet++ & 32.59 & 70.25 & 84.93 & 87.11 & 0 & 0.99 & 3.39 & 5.73   \\
   % Graphormer3D & — & — & 9.17 & 21.82 & 0 & 0 & 0 & 0   \\
  %  GemNet-OC & 69.38 & 81.59 & 83.71 & \textbf{89.58} & 0.25 & 1.05 & 1.6 & 9.2  \\
 %   EquiformerV2 & 65.85 & 74.12 & 76.15 & 81.95 & 1 & 2.65 & 2.8 & 3.85\\
%    eSCN & \textbf{82.31} & \textbf{86.2} & \textbf{87.28} & 88.67 & \textbf{1.9} & \textbf{4.25} & \textbf{5.25} & 7.9   \\
    % \hline
%    \hline 
%\end{tabular*}
%\label{tbl:optimization_results}
%\end{table*}
%\begin{table*}[!t]
%\caption{The $\overline{\operatorname{pct}_{div}}$  for the geometry optimization task}
%\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}|l|P{.07\linewidth}|P{.07\linewidth}|P{.07\linewidth}|P{.07\linewidth}|}
%    \hline
%
%    \multirow{2}{*}{\textbf{Model}} &
%      \multicolumn{4}{c|}{$\displaystyle \overline{\operatorname{pct}}_{div}(\%)\downarrow$} \\
%    & $\mathcal{D^{\text{tiny}}}$ & $\mathcal{D^{\text{small}}}$ & $\mathcal{D^{\text{medium}}}$ & $\mathcal{D^{\text{large}}}$ \\
%      \hline 
%    SchNet & 8.45 & 4.05 & 3.5 & 0.1   \\
    % \hline
%    PaiNN & $\textbf{2.15}$ & $\textbf{3.}$ & 3.4 & $\textbf{0.05}$    \\
%    DimeNet++ & 97.08 & 4.58 & $\textbf{1.72}$ & 0.42    \\
%    Graphormer3D & 100 & 100 & 99.95 & 99.45 \\
%    GemNet-OC & 26.55 & 13.35 & 19.90 & 0.35  \\
%    EquiformerV2 & 56.45 & 45.29 & 48.80 & 49.30\\
%    eSCN & 21.85 & 8.35 & 1.75 & 0.2   \\
    % \hline
%    \hline 
%\end{tabular*}
%\label{tbl:optimization_results_div}

%\end{table*}


% \begin{table}[ht]
% %\setstretch{0.9}
% \caption{The $\overline{\operatorname{pct}_{div}}$  for the geometry optimization task}
% \vspace{-0.3cm}
% \begin{center}
% \begin{small}
% \begin{tabular}{l|cccc}

% \multirow{2}{*}{\textbf{Model}} &
%       \multicolumn{4}{c}{$\displaystyle \overline{\operatorname{pct}}_{div}(\%)\downarrow$} \\
%     & $\mathcal{D^{\text{tiny}}}$ & $\mathcal{D^{\text{small}}}$ & $\mathcal{D^{\text{medium}}}$ & $\mathcal{D^{\text{large}}}$ \\
%       \toprule 
%     SchNet & 8.45 & 4.05 & 3.5 & 0.1   \\
%     % \hline
%     PaiNN & $\textbf{2.15}$ & $\textbf{3.}$ & 3.4 & $\textbf{0.05}$    \\
%     DimeNet++ & 97.08 & 4.58 & $\textbf{1.72}$ & 0.42    \\
%     Graphormer3D & 100 & 100 & 99.95 & 99.45 \\
%     GemNet-OC & 26.55 & 13.35 & 19.90 & 0.35  \\
%     EquiformerV2 & 56.45 & 45.29 & 48.80 & 49.30\\
%     eSCN & 21.85 & 8.35 & 1.75 & 0.2   \\
%     % \hline
%     \bottomrule 

% \end{tabular}
% \end{small}

% \end{center}
% \label{tbl:optimization_results_div}
% \end{table}

% \begin{table}[!t]\centering\small
% %\setstretch{0.9}
% \caption{The $\overline{\operatorname{pct}_T}$ and $\operatorname{pct}_{\text{success}}$ for the geometry optimization task.} %\label{tbl:optimization_results}

% \begin{tabular}{l|cccc|cccc}
% \toprule
% \multirow{2}{*}{\textbf{Model}} &
%       \multicolumn{4}{c|}{$\displaystyle \overline{\operatorname{pct}}_T(\%)\uparrow$} &
%       \multicolumn{4}{c}{$\operatorname{pct}_{\text{success}}(\%) \uparrow$ }\\
%     &$\mathcal{D^{\text{tiny}}}$ & $\mathcal{D^{\text{small}}}$ & $\mathcal{D^{\text{medium}}}$ & $\mathcal{D^{\text{large}}}$ & $\mathcal{D^{\text{tiny}}}$ & $\mathcal{D^{\text{small}}}$ & $\mathcal{D^{\text{medium}}}$ & $\mathcal{D^{\text{large}}}$\\
%       \midrule 
%     SchNet & 61.35 & 65.00 & 61.10 & 80.82 & 0 & 0 & 0 & 1.15   \\
%     % \hline
%     PaiNN & 69.31 & 73.66 & 76.99 & 89.40 & 0 & 0.15 & 1.00 & \textbf{11.05}   \\
%     DimeNet++ & 32.59 & 70.25 & 84.93 & 87.11 & 0 & 0.99 & 3.39 & 5.73   \\
%     Graphormer3D & — & — & 9.17 & 21.82 & 0 & 0 & 0 & 0   \\
%     GemNet-OC & 69.38 & 81.59 & 83.71 & \textbf{89.58} & 0.25 & 1.05 & 1.6 & 9.2  \\
%     EquiformerV2 & 65.85 & 74.12 & 76.15 & 81.95 & 1 & 2.65 & 2.8 & 3.85\\
%     eSCN & \textbf{82.31} & \textbf{86.2} & \textbf{87.28} & 88.67 & \textbf{1.9} & \textbf{4.25} & \textbf{5.25} & 7.9   \\
%     % \hline 
%     \bottomrule 
% \end{tabular}
% \end{table}



==> tables/summary_datasets.tex <==
\begin{table}[!t]
\caption{Summary of quantum chemistry datasets; $\ast$~-- not provided directly but can be derived.}\label{tbl:dataset-summary} 
% (+) denotes information that is not provided in a direct way in article or descriptions. (*) denotes parameters that can be derived from dataset with some computation.}
\scriptsize\setlength{\tabcolsep}{1.5pt}
\def\mytabwid{.08\linewidth}
\def\mytabwidd{.11\linewidth}
\begin{tabular}{L{\mytabwidd}L{\mytabwidd}L{\mytabwidd}L{\mytabwid}L{\mytabwid}L{\mytabwid}L{\mytabwid}L{\mytabwidd}L{\mytabwid}L{\mytabwid}} \toprule
& \textbf{$\nabla^2$DFT} & \textbf{$\nabla$DFT} & \textbf{QM7} & \textbf{QM7b} & \textbf{QM7-X} & \textbf{QM9} & \textbf{MultiXC-QM9} & \textbf{QM1B} & \textbf{QH9} \\\midrule
Chem. inf. source & MOSES, ZINC21 (Zinc Clean Leads) & MOSES, ZINC21 (Zinc Clean Leads) & GDB-13                                                                                      & GDB-13                                                                                          & GDB-13                                                                                  & GDB-17                                                                                  & GDB-17                                                                                   & GDB-11                                                                 & GDB-13, QM9                          \\
\# mole\-cules    & 2M                                                                               & 1M                                                                                 & 7K                                                                                          & 7K                                                                                              & 7K                                                                                      & 134K                                                                                    & 134K                                                                                     & 1M                                                                     & 130K                                                                                              \\
\# con\-for\-mers      & 13M                                                                              & 5M                                                                                 & 7K                                                                                          & 7K                                                                                              & 4M                                                                                      & 134K                                                                                    & 134K                                                                                     & 1B                                                                     & 130K                                                                                              \\
\# atoms             & 8-62                                                                             & 8–62                                                                               & 1-23                                                                                        & 1-23                                                                                            & 1-23                                                                                    & 3-29                                                                                    & 3-29                                                                                     & 9-11                                                                   & 3-29                                                                                              \\
\# heavy atoms    & 8-27                                                                             & 8–27                                                                               & 1-7                                                                                         & 1-7                                                                                             & 1-7                                                                                     & 1-9                                                                                     & 1-9                                                                                      & --- & 1-9 \\
Atoms                                                              & H,C,N,O,S, Cl,F,Br                 & H,C,N,O, Cl,F,Br                      & H,C,N,O,S                                        & H,C,N,O,S                                            & H,C,N,O, S,Cl                                 & H,C,N,O,F                                    & H,C,N,O,F                                     & H,C,N,O,F                   & H,C,N,O,F            \\
                                  Forces             & Yes                                                                              & Yes                                                                                & No                                                                                          & No                                                                                              & Yes                                                                                     & No                                                                                      & No                                                                                       & No                                                                     & Yes                                                                                               \\
Hamil\-to\-ni\-ans                                                   & Yes                                                                              & Yes                                                                                & No                                                                                          & No                                                                                              & No                                                                                      & No                                                                                      & No                                                                                       & No                                                                     & No                                                                                                \\
Optim. traj.              & Yes                                                                              & No                                                                                 & No                                                                                          & No                                                                                              & No                                                                                      & No                                                                                      & No                                                                                       & No                                                                     & Yes                                                                                               \\
Basis set and XC-func. & $\Omega$B97X- D/ Def2- SVP         & $\Omega$B97X- D/ Def2- SVP           & PBE0                                                                                        & ZINDO,  SCS,  PBE0,  GW                           & ePBE0+ MBD,  TotFOR                         & B3LYP/6- 31G(2df,p) + G4MP2                 & B3LYP,PBE/ 6–31G(2df,p), SZ,DZP,TZP & STO-3G/ B3LYP  & B3LYP/ Def2SVP \\
Storage size             & 220 Tb                                                                           & 100 Tb                                                                             & 17.9 MB                                                                                     & 16.1 MB                                                                                         & 1.35 Gb                                                                                 & 230 Mb                                                                                  & 317 Gb                                                                                   & 240 GB                                                                 & 28.4 Gb                                                                                           \\ \midrule
                                                                   & \textbf{GEOM}                                                                    & \textbf{ANI-1}                                                                     & \textbf{ANI-1x/ ANI-1cxx}                         & \textbf{OrbNet Denali}                                & \textbf{QMugs}                                                                          & \textbf{SPICE}                                                                          & \textbf{PubChemQC}                                                                       & \textbf{Frag20}                                                        & \textbf{VQM24}                                                                                    \\ \hline
Chem. inf. source        & QM9, AICures                           & GDB                                                                                & GDB-11, ChEMBL                                    & ChEM- BL27                                                                                        & ChEMBL                                                                                  & {\tiny PubChem+, DES370K+, other}                     & PubChem                                                                                  & PubChem, ZINC                & {Combi\-na\-to\-rial}                               \\
\# molecules          & 450K                                                                             & 57K                                                                                & 57K                                                                                         & 16K                                                                                             & 665K                                                                                    & 19K                                                                                     & 85M                                                                                      & 565K                                                                   & 10K                                                                                               \\
\# conformers        & 37M                                                                              & 24M                                                                                & 20M                                                                                         & 2.3M                                                                                            & 2M                                                                                      & 1KK                                                                                     & 85M                                                                                      & 566K                                                                   & 835K                                                                                              \\
\# atoms             & ---                                                                                & ---                                                                                  & 2-26                                                                                        & ---                                                                                               & 4-228                                                                                   & 2–96                                                                                    & ---                                                                                        & ---                                                                      & 4,5                                                                                               \\
\# heavy  atoms    & ---                                                                                & 1-11                                                                               & 1-8                                                                                         & ---                                                                                               & 4-100                                                                                   & ---                                                                                       & 51                                                                                       & 20                                                                     & ---                                                                                         \\
Atoms                                                              & H,C,N,O,F,+                           & H,C,N,O                                 & H,C,N,O                                          & H,Li,B,C, N,O,F,Na, Mg,Si,P,S, Cl,K,Ca,Br,I & H,C,N,O, P,S,Cl,F, Br,I                  & H,Li,C,N, O,F,Na,Mg, P,S,Cl,K, Ca,Br,I & H,C,N, O,P,S, F,Cl,Na, K,Mg,Ca           & H,B,C,O, N,F,P, S,Cl,Br & H,C,N,O, F,Si,P, S,Cl,Br                           \\
Forces             & Yes                                                                              & No                                                                                 & No                                                                                          & No                                                                                              & No*                                                                                     & Yes                                                                                     & No                                                                                       & No                                                                     & No                                                                                                \\
Hamiltonians         & No                                                                               & No                                                                                 & No                                                                                          & No                                                                                              & No*                                                                                     & No                                                                                      & No                                                                                       & No                                                                     & No                                                                                                \\
Optim traj.              & No                                                                               & No                                                                                 & No                                                                                          & No                                                                                              & No                                                                                      & No                                                                                      & No                                                                                       & No                                                                     & No                                                                                                \\
Basis set and XC-func. & mTZVPP/ R2scan-3                       & WB97x/ 6–31g(d)                          & {\tiny wB97x/6-31G*,  wB97x/ def2-TZVPP,  CCSD(T)*/ CBS} & $\Omega$B97X- D3/ Def2- TZVP                      & {\tiny $\omega$B97X- D/ Def2- SVP +GFN2- XTB} & {\tiny $\omega$B97M- D3(BJ)/ Def2- TZVPPD}        & B3LYP/ 6-31G*+ PM6                           & B3LYP/ 6-31G*                & {\tiny $\Omega$B97X-D3/ Cc- pVDZ, DMC@ PBE0(cEC/ Cc-VQZ))} \\
Storage size             & 130.8 GB                                                                         & 4.48 Gb                                                                            & 5.29 Gb                                                                                     & 2.74 GB                                                                                         & 7 Tb                                                                                    & 37.5 GB                                                                                 & 100 Tb                                                                                   & 566 Mb                                                                 & 1.5 Gb                                                                                  \\\bottomrule    
\end{tabular}
\end{table}

